Adaptive Ranking Based Constraint Handling for Explicitly Constrained Black-Box Optimization

We propose a novel constraint-handling technique for the covariance matrix adaptation evolution strategy (CMA-ES). The proposed technique is aimed at solving explicitly constrained black-box continuous optimization problems, in which the explicit constraint is a constraint whereby the computational time for the constraint violation and its (numerical) gradient are negligible compared to that for the objective function. This method is designed to realize two invariance properties: invariance to the affine transformation of the search space, and invariance to the increasing transformation of the objective and constraint functions. The CMA-ES is designed to possess these properties for handling difficulties that appear in black-box optimization problems, such as non-separability, ill-conditioning, ruggedness, and the different orders of magnitude in the objective. The proposed constraint-handling technique (CHT), known as ARCH, modifies the underlying CMA-ES only in terms of the ranking of the candidate solutions. It employs a repair operator and an adaptive ranking aggregation strategy to compute the ranking. We developed test problems to evaluate the effects of the invariance properties, and performed experiments to empirically verify the invariance of the algorithm. We compared the proposed method with other CHTs on the CEC 2006 constrained optimization benchmark suite to demonstrate its efficacy. Empirical studies reveal that ARCH is able to exploit the explicitness of the constraint functions effectively, sometimes even more efficiently than an existing box-constraint handling technique on box-constrained problems, while exhibiting the invariance properties. Moreover, ARCH overwhelmingly outperforms CHTs by not exploiting the explicit constraints in terms of the number of objective function calls.

==> header.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[utf8]{inputenc}

% For japanese typeset
\usepackage{amsmath,amsthm,amssymb} %% needed explicitely for org-preview-latex
\usepackage{subcaption}
\usepackage{mathtools}
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{braket}
\usepackage{stmaryrd}        % \llbracket, \rrbracket
\usepackage{xcolor,hyperref}
% \usepackage[dvipdfmx]{xcolor}
\usepackage{cleveref}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Algorithmic environment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[linesnumbered,boxed,vlined,ruled]{algorithm2e}
\DontPrintSemicolon
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\SetKwRepeat{Repeat}{repeat}{until}

\SetStartEndCondition{ }{}{}%
\SetKwProg{Fn}{def}{\string:}{}
\SetKwIF{If}{ElseIf}{Else}{if}{:}{else if}{else:}{}%
\SetKw{KwTo}{in}\SetKwFor{For}{for}{\string:}{}%
\SetKwFor{While}{while}{:}{fintq}%
\SetKw{KwRet}{return}
\SetKw{Return}{return}


\SetKwFunction{ComputeGradient}{ComputeGradient}
\SetKwFunction{ComputeDescentDirection}{ComputeDescentDirection}
\SetKwFunction{Resample}{Resample}
\SetKwFunction{Concatenate}{Concatenate}
\SetKwFunction{UpdateDBusing}{UpdateDBusing}
\SetKwFunction{SampleFromDB}{SampleFromDB}
\SetKwFunction{RandomSelect}{RandomSelect}
\SetKwFunction{LabelingDBusing}{LabelingDBusing}


\makeatletter
\newenvironment{algoproc}[1][]
  {\renewcommand{\algorithmcfname}{Procedure}%
   \begin{algorithm}[#1]
   \long\def\@caption##1[##2]##3{%
     \par
     \begingroup\@parboxrestore
     \if@minipage\@setminipage\fi
     \normalsize \@makecaption{\AlCapSty{\AlCapFnt\algorithmcfname}}{\ignorespaces ##3}%
     \par\endgroup
   }}
  {\end{algorithm}}
\makeatother

\makeatletter
\newenvironment{algofunc}[1][]
  {\renewcommand{\algorithmcfname}{Function}%
   \begin{algorithm}[#1]
   \long\def\@caption##1[##2]##3{%
     \par
     \begingroup\@parboxrestore
     \if@minipage\@setminipage\fi
     \normalsize \@makecaption{\AlCapSty{\AlCapFnt\algorithmcfname}}{\ignorespaces ##3}%
     \par\endgroup
   }}
  {\end{algorithm}}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% bibtex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[backend=biber, style=numeric]{biblatex}
\DeclareSortingTemplate{mysorting}{
  \sort{\citeorder}
  \sort{
    \field{sortname}
    \field{author}
    \field{editor}
  }
  \sort{
    \field{sortyear}
    \field{year}
  }
  \sort[direction=descending]{
    \field{sorttitle}
    \field{title}
  }
}
\ExecuteBibliographyOptions{sorting=mysorting}

\addbibresource{/Users/naoki/drive/github.com/akimotolab/trunk/publication/ref.bib}
\addbibresource{/Users/naoki/drive/github.com/akimotolab/trunk/reference/ref.bib}
\addbibresource{/Users/naoki/org/braindump/org/preferences/ref.bib}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Displays
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifx\theorem\undefined{\newtheorem{theorem}{Theorem}}\fi
\ifx\proposition\undefined{\newtheorem{proposition}{Proposition}}\fi
\ifx\corollary\undefined{\newtheorem{corollary}{Corollary}}\fi
\ifx\lemma\undefined{\newtheorem{lemma}{Lemma}}\fi

\ifx\definition\undefined{\newtheorem{definition}{Definition}}\fi
\ifx\example\undefined{\newtheorem{example}{Example}\renewcommand\theexample{\unskip}}\fi
\ifx\assumption\undefined{\newtheorem{assumption}{Assumption}}\fi

\ifx\remark\undefined{\newtheorem{remark}{Remark}\renewcommand\theremark{\unskip}}\fi

\crefname{table}{Table}{Tables}
\crefname{figure}{Figure}{Figures}
\crefname{section}{Section}{Sections}
\crefname{equation}{Eq}{Eqs}
\crefname{definition}{Definition}{Definitions}
\crefname{theorem}{Theorem}{Theorems}
\crefname{proposition}{Proposition}{Propositions}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{proposition}{Proposition}{Propositions}
\crefname{algorithm}{Algorithm}{Algorithms}
\crefname{example}{Example}{Examples}
\crefname{remark}{Remark}{Remarks}
\crefname{assumption}{Assumption}{Assumptions}
\renewcommand{\figurename}{Figure }
\renewcommand{\tablename}{Table }
% \usepackage{geometry}
% \geometry{left=25mm,right=25mm,top=30mm,bottom=30mm}

%%% JA
% \newcommand*{\exclamationmark}[1]
%             {\tikz\node{\fontfamily{LinuxLibertineT-LF}\fontsize{2.5em}{2.5ex}\selectfont\textbf{!}};}
% \definecolor{todoshade}{rgb}{1,0.95,0.95}
% \newenvironment{todo}{%
%   \def\FrameCommand{%
%     \noindent\hspace{1em}%
%     {\color{borderline}\vrule width 0.3em}%
%     {\color{todoshade}\vrule width 0.5em}%
%     \colorbox{todoshade}%
%   }%
%   \MakeFramed{\advance\hsize-\width\FrameRestore}%
%   \vspace{-3ex}%
%   \noindent\exclamationmark%
%   \noindent\hspace{-10em}% disable indenting first paragraph
%   \begin{adjustwidth}{}{-1.8em}%
% }
% {%
%   \vspace{3ex}\end{adjustwidth}\endMakeFramed%
% }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% My Commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\eps}{\varepsilon}
\newcommand{\card}{\mathtt{Card}}
\newcommand{\nq}{N_\eps (q)}
\newcommand{\np}{N_\eps (p)}
\newcommand{\pt}{\mathrm{MinPts}}
\renewcommand{\geq}{\geqslant} % geq
\renewcommand{\leq}{\leqslant} % leq
\newcommand{\OO}{\mathcal{O}}
\newcommand{\NN}{\mathcal{N}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\XX}{\mathbb{X}}
\DeclarePairedDelimiterX{\inner}[2]{\langle}{\rangle}{#1, #2}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\providecommand{\argmax}{\operatornamewithlimits{argmax}} % argmax
\providecommand{\argmin}{\operatornamewithlimits{argmin}} % argmin
\newcommand{\mpts}{m_\mathrm{pts}}
\newcommand{\Gm}{G_\mpts}
\newcommand{\mcs}{m_\mathrm{clSize}}
\newcommand{\feas}{\mathrm{feas}}
\newcommand{\xfeas}{x^\feas}
\newcommand{\T}{\mathrm{T}}
\newcommand{\Gtheta}{G_\theta}
\newcommand{\dbf}{\mathrm{DB}^\feas}
\newcommand{\tmp}{\mathrm{tmp}}
\newcommand{\dbt}{\mathrm{DB}^\tmp}

